Dietcoin: shortcutting the Bitcoin verification process for your smartphone

Blockchains have a storage scalability issue. Their size is not bounded and they grow indefinitely as time passes. As of August 2017, the Bitcoin blockchain is about 120 GiB big while it was only 75 GiB in August 2016. To benefit from Bitcoin full security model, a bootstrapping node has to download and verify the entirety of the 120 GiB. This poses a challenge for low-resource devices such as smartphones. Thankfully, an alternative exists for such devices which consists of downloading and verifying just the header of each block. This partial block verification enables devices to reduce their bandwidth requirements from 120 GiB to 35 MiB. However, this drastic decrease comes with a safety cost implied by a partial block verification. In this work, we enable low-resource devices to fully verify subchains of blocks without having to pay the onerous price of a full chain download and verification; a few additional MiB of bandwidth suffice. To do so, we propose the design of diet nodes that can securely query full nodes for shards of the UTXO set, which is needed to perform full block verification and can otherwise only be built by sequentially parsing the chain.

==> Makefile <==
.PHONY: all clean html dvi dvi-lazy pdf pdf-lazy ps rtf text viewpdf viewdvi

LATEX        = latex
PDFLATEX     = pdflatex
TARGET       = RR-9162
SOURCE_FILES = $(TARGET).tex $(wildcard dietcoin*.tex) $(wildcard algos/*.tex) revision_macros.tex
PS2PDF       = ps2pdf -sPAPERSIZE=letter
FIGURES      = figs/BitcoinExplanationsFrancois_AddingTransaction_cropped.pdf\
               figs/BitcoinExplanationsFrancois_Overview_cropped.pdf\
               figs/BitcoinExplanationsFrancois_HijackingAttempt_cropped.pdf\
               figs/BitcoinExplanationsFrancois_BranchedChain_cropped.pdf\
               figs/BitcoinExplanationsFrancois_StuctureTransaction_cropped.pdf\
               figs/BitcoinExplanationsFrancois_Chaining_cropped.pdf
# $(wildcard ../figs/*.{pdf,png,jpg}) # $(wildcard ../figs/*.png) $(wildcard fig/*.jpg)
BIB_FILES    = $(wildcard *.bib)

# Set the pdf reader according to the operating system
OS = $(shell uname)
ifeq ($(OS), Darwin)
	PDF_READER = open
endif
ifeq ($(OS), Linux)
	PDF_READER = evince
endif

all: pdf

pdf-lazy:
	make $(FIGURES)
	-bibtex $(TARGET)
	$(PDFLATEX) --jobname=$(TARGET) $(SOURCE_FILES) > /dev/null
	$(PDF_READER) $(TARGET).pdf
	-bibtex $(TARGET)
#	$(LATEX) $(TARGET).tex
#	bibtex $(TARGET)

$(TARGET).pdf: $(SOURCE_FILES) $(BIB_FILES) $(FIGURES)
	$(PDFLATEX) --jobname=$(TARGET) $(SOURCE_FILES)
	-bibtex $(TARGET)
	$(PDFLATEX) --jobname=$(TARGET) $(SOURCE_FILES) # Bibtex ne marche pas sinon (!)
	$(PDFLATEX) --jobname=$(TARGET) $(SOURCE_FILES) # Bibtex ne marche pas sinon (!)

pdf: $(TARGET).pdf

text: $(TARGET).pdf
	pdftotext $(TARGET).pdf

viewpdf: pdf
	$(PDF_READER) $(TARGET).pdf &

html:
	latex2html -no_transparent -no_navigation -math -split 0 -noimages -noantialias $(TARGET).tex

rtf:
	latex2rtf $(TARGET).tex

../figs/%.eps: ../figs/%.plot
	cd figs; gnuplot $(notdir $<)

../figs/%_cropped.pdf: ../figs/%.pdf
	pdfcrop $< $@

clean:
	rm -f $(TARGET).ps $(TARGET).pdf $(TARGET).synctex.gz *.dvi *.aux *.bbl *.blg *.toc *.ind *.out *.brf *.ilg *.idx *.log


==> dietcoin_algos.tex <==
% -*- tex-main-file: "RR-9162" compile-command: "make pdf" ispell-dictionary: "american" -*

% \input{algos/algo_include}
\input{../algos/algo_tables}
\input{../algos/algo_common}
% \input{algos/algo_spv_compact}
\input{../algos/algo_spv}
\input{../algos/algo_full_node}
\input{../algos/algo_miner}

%%% Local Variables:
%%% mode: latex
%%% End:

